Extending Complex Logical Queries on Uncertain Knowledge Graphs

The study of machine learning-based logical query answering enables reasoning with large-scale and incomplete knowledge graphs. This paper advances this area of research by addressing the uncertainty inherent in knowledge. While the uncertain nature of knowledge is widely recognized in the real world, it does not align seamlessly with the first-order logic that underpins existing studies. To bridge this gap, we explore the soft queries on uncertain knowledge, inspired by the framework of soft constraint programming. We propose a neural symbolic approach that incorporates both forward inference and backward calibration to answer soft queries on large-scale, incomplete, and uncertain knowledge graphs. Theoretical discussions demonstrate that our method avoids catastrophic cascading errors in the forward inference while maintaining the same complexity as state-of-the-art symbolic methods for complex logical queries. Empirical results validate the superior performance of our backward calibration compared to extended query embedding methods and neural symbolic approaches.

==> table.tex <==
\begin{table*}
\scriptsize
\centering
\caption{Result of answering soft queries. % compare our methods with query embedding, including LogicE and ConE.  
%on three graphs across 11 query types and four metrics. 
Logic+NE and ConE+NE refer to the query embedding with number embedding extensions. SRC is our inference method, and SRC(D), SRC(L), and SRC(D+L) is explained in Section~\ref{sec:calibration}.}
\label{Main result}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}cccccccccccccccccc@{}}
\toprule
\multirow{2}{*}{uncertain KG}      & \multirow{2}{*}{Models} & \multicolumn{13}{c}{$\tau$}                                                                            & \multirow{2}{*}{AVG. $\rho$} & \multirow{2}{*}{AVG. MAP} & \multirow{2}{*}{AVG. NDCG} \\ \cmidrule(lr){3-15}
                          &                     & 1P   & 2P   & 2I   & 2IN  & 2IL  & 2M   & 2U    & 3IN  & IP   & IM   & INP  & UP   & AVG.           &                         &                      &                       \\ \midrule
\multirow{4}{*}{CN15k}    & LogicE+NE              & 9.1  & -1.5 & 4.8  & 6.0  & 18.3 & 5.1  & -14.1 & 3.5  & -2.4 & 6.4  & -0.9 & 9.6  & 4.8           & 5.8                     & 7.0                  & 11.2                  \\
                          & ConE+NE               & 5.3  & 4.3  & 3.5  & 6.3  & 18.4 & 6.9  & 20.5  & 2.9  & 1.8  & 10.4 & 1.7  & 14.9 & 8.1           & 10.0                    & 7.7                  & 13.2                  \\
& SRC                 & 15.0 & 2.4  & -0.0 & 2.1  & 10.7 & 9.2  & 25.5  & -2.0 & -9.0 & 7.9  & -4.4 & 13.0 & 5.9           & 8.9                     & 9.2                  & 15.5                  \\
& SRC(D)           & 16.6&11.8&-0.6&6.9&10.9&11.7&34.4&0.1&5.2&12.5&4.7&24.2&11.5 & 15.1    & 12.9        & 21.8 \\
& SRC(L) & 15.8 & 11.8 & -0.4 & 2.4  & 11.0 & 12.4 & 32.3  & -0.8 & 3.6  & 11.1 & 1.1  & 22.8 & 10.3 & 13.7           & 12.6        & 21.1         \\ 
& SRC(D+L)           & 15.6&13.4&-0.3&5.2&11.2&13.5&36.8&-0.4&8.2&12.2&4.8&28.2&\textbf{12.4} & \textbf{16.2}           & \textbf{13.7}        & \textbf{23.2}         \\ 
                            \midrule
\multirow{4}{*}{PPI5k}    & LogicE+NE              & 20.5 & 22.6 & 17.1 & 10.4 & 24.4 & 20.0 & 30.4  & 9.1  & 12.4 & 14.1 & -2.6 & 32.9 & 14.8          & 20.7                    & 8.0                  & 16.4                  \\
                          & ConE+NE              & 29.2 & 42.5 & 26.4 & 20.7 & 32.6 & 33.9 & 35.9  & 16.6 & 36.6 & 29.4 & 22.5 & 42.2 & 30.7          & 40.8                    & 44.1                 & 49.2                  \\
& SRC                 & 66.6 & 70.9 & 49.9 & 42.7 & 71.0 & 42.9 & 71.6  & 32.7 & 65.6 & 37.1 & 57.2 & 70.4 & 56.5          & 66.7                    & 68.4                 & 70.7                  \\
& SRC(D)           & 66.7&68.7&53.1&44.9&73.1&46.7&73.3&37.7&63.7&41.3&56.9&69.9&58.0& 68.5    & 64.0        & 69.8 \\

& SRC(L)            & 66.8 & 71.7 & 52.7 & 43.4 & 72.8 & 43.8 & 72.7  & 34.4 & 66.6 & 38.3 & 58.0 & 71.4 & 57.7 & 67.8           & \textbf{69.8}        & \textbf{71.6}         \\ 
& SRC(D+L)           & 66.9&69.0&53.5&45.1&73.5&46.9&73.4&38.1&63.8&41.6&57.1&69.9&\textbf{58.2}& \textbf{68.7}    & 64.1       & 70.1 \\ 
                                                      \midrule
\multirow{4}{*}{O*NET20k} & LogicE+NE              & 6.3  & 9.5  & 43.5 & 3.9  & 36.6 & 9.7  & 15.3  & 8.3  & 11.1 & 8.8  & 3.8  & -9.8 & 13.8          & 18.5                    & 3.5                  & 6.4                   \\
                          & ConE+NE                 & 30.8 & 41.9 & 57.0 & 21.8 & 46.0 & 37.7 & 49.7  & 48.0 & 22.7 & 21.7 & 14.2 & 53.1 & 36.8          & 47.2                    & 27.5                 & 38.7                  \\
& SRC                 & 72.0 & 54.9 & 68.6 & 67.6 & 67.3 & 36.9 & 76.0  & 59.2 & 47.6 & 29.1 & 48.9 & 52.4 & 57.3          & 65.3                    & 27.1                 & 41.3                  \\
& SRC(D)           & 71.7&55.2&74.3&67.7&70.9&49.3&80.1&65.0&52.7&44.7&48.9&55.4&61.8& 70.2    & 26.6        & 41.5 \\
& SRC(L)             & 71.6 & 56.7 & 69.8 & 66.8 & 68.4 & 38.2 & 77.6  & 59.9 & 51.3 & 32.1 & 49.8 & 55.4 & 58.7 & 66.5           & \textbf{27.6}        & \textbf{41.8}         \\ 
& SRC(D+L)           & 71.7&55.6&74.3&67.5&71.0&49.7&80.2&65.0&52.9&45.2&49.2&55.9&\textbf{61.9}& \textbf{70.5}    & 26.7    & 41.7 \\
                       \bottomrule
\end{tabular}}
\end{table*}
